Bespoke Non-Stationary Solvers for Fast Sampling of Diffusion and Flow Models

This paper introduces Bespoke Non-Stationary (BNS) Solvers, a solver distillation approach to improve sample efficiency of Diffusion and Flow models. BNS solvers are based on a family of non-stationary solvers that provably subsumes existing numerical ODE solvers and consequently demonstrate considerable improvement in sample approximation (PSNR) over these baselines. Compared to model distillation, BNS solvers benefit from a tiny parameter space ($<$200 parameters), fast optimization (two orders of magnitude faster), maintain diversity of samples, and in contrast to previous solver distillation approaches nearly close the gap from standard distillation methods such as Progressive Distillation in the low-medium NFE regime. For example, BNS solver achieves 45 PSNR / 1.76 FID using 16 NFE in class-conditional ImageNet-64. We experimented with BNS solvers for conditional image generation, text-to-image generation, and text-2-audio generation showing significant improvement in sample approximation (PSNR) in all.

==> algorithms/general_solver.tex <==
\begin{wrapfigure}[7]{R}{0.3\textwidth}
\vspace{-23pt}
\resizebox{0.289\textwidth}{!}{
    \begin{minipage}{0.37\textwidth}
      \begin{algorithm}[H]
        \caption{Numerical ODE solver.}\label{alg:odesolve}
        \begin{algorithmic}
            \Require $x_0,\ f$
            %\State {\small \color{gray} \% Sequential for loop over steps}
            \State $X_{-1} \gets \begin{bmatrix}\end{bmatrix}$
            \State $F_{-1} \gets \begin{bmatrix}\end{bmatrix}$
            \For{$i=0,1,\ldots,n-1$}
            \State $X_i = \begin{bmatrix}X_{i-1} & x_{t_i}\end{bmatrix}$
            \State $F_i = \begin{bmatrix}F_{i-1} & f_{t_i}(x_{t_i})\end{bmatrix}$
            \State $x_{t_{i+1}} = \odestep_i(T_n, X_i, F_i)$  
        \EndFor
        \State \Return $x_n$
        \end{algorithmic}
      \end{algorithm}
    \end{minipage} }
  \end{wrapfigure}

==> tables/eponential_exact_solution_coffeicients.tex <==
\begin{wraptable}[10]{r}{0.125\textwidth}
% \vspace{-10pt}
% \hspace{-15pt}
\setlength{\tabcolsep}{2.0pt}
\centering
\resizebox{0.125\textwidth}{!}{
    \begin{tabular}{lcc} 
     %\Xhline{1pt} %\hline 
     % \toprule
       $f$ &  $\psi$ & $y$ \\ \midrule %\Xhline{1pt}
      $\eps$-pred & $\alpha_t$ & $-1$\\ 
      $x$-pred & $\sigma_t$ & $1$\\ \midrule
     %\Xhline{1pt} 
     \bottomrule  
    \end{tabular}
} 
\caption{XXX}\label{tab:exp_exact_sol_coefficients}
\end{wraptable} 

==> tables/times.tex <==
\begin{wraptable}[20]{r}{0.44\textwidth}\vspace{-10pt}
\setlength{\tabcolsep}{2.0pt}
\centering
\resizebox{0.43\textwidth}{!}{
\begin{tabular}{lccccc} 
 %\Xhline{1pt} %\hline 
 \toprule
  & NFE & ImageNet 64 & ImageNet 128 & Shutterstock 512 & Audio \\ \midrule %\Xhline{1pt}
 \textbf{\textit{Training times}}
 &
 \begin{tabular}[t]{c}
       4 \\ 6 \\ 8 \\ 10 \\ 12 \\ 14 \\ 16 \\18 \\ 20
 \end{tabular}
 & 
 \begin{tabular}[t]{c}
      XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\
 \end{tabular}
 &
 \begin{tabular}[t]{c}
      XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\
 \end{tabular}  
 &
 \begin{tabular}[t]{c}
      - \\ - \\ XXX \\ - \\ XXX \\ - \\ XXX \\ - \\ XXX \\
 \end{tabular} 
 &
 \begin{tabular}[t]{c}
      XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\ XXX \\
 \end{tabular} \\[35pt]
 % %
 % %
 % %
\bottomrule  
\end{tabular}
}\vspace{-5pt}
\caption{
Training times of BNS.
}\label{tab:times}
\end{wraptable} 


\begin{wraptable}[20]{r}{0.44\textwidth}\vspace{-10pt}
\setlength{\tabcolsep}{2.0pt}
\centering
\resizebox{0.43\textwidth}{!}{
\begin{tabular}{lccccccccc} 
 %\Xhline{1pt} %\hline 
 \toprule
  NFE: & 4 & 6 & 8 & 10 & 12 & 14 & 16 &1 8 & 20 \\ \midrule %\Xhline{1pt}
 \textbf{\textit{ImageNet 64}}
 & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
 \textbf{\textit{ImageNet 128}}
 & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
 \textbf{\textit{Shutterstock 512}}
 & - & - & XXX & - & XXX & - & XXX & - & XXX \\
 \textbf{\textit{Audio}}
 & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
 % %
 % %
 % %
\bottomrule  
\end{tabular}
}\vspace{-5pt}
\caption{
Training times of BNS.
}\label{tab:shutterstock}
\end{wraptable} 
